Spiking Vision Transformer with Saccadic Attention

The combination of Spiking Neural Networks (SNNs) and Vision Transformers (ViTs) holds potential for achieving both energy efficiency and high performance, particularly suitable for edge vision applications. However, a significant performance gap still exists between SNN-based ViTs and their ANN counterparts. Here, we first analyze why SNN-based ViTs suffer from limited performance and identify a mismatch between the vanilla self-attention mechanism and spatio-temporal spike trains. This mismatch results in degraded spatial relevance and limited temporal interactions. To address these issues, we draw inspiration from biological saccadic attention mechanisms and introduce an innovative Saccadic Spike Self-Attention (SSSA) method. Specifically, in the spatial domain, SSSA employs a novel spike distribution-based method to effectively assess the relevance between Query and Key pairs in SNN-based ViTs. Temporally, SSSA employs a saccadic interaction module that dynamically focuses on selected visual areas at each timestep and significantly enhances whole scene understanding through temporal interactions. Building on the SSSA mechanism, we develop a SNN-based Vision Transformer (SNN-ViT). Extensive experiments across various visual tasks demonstrate that SNN-ViT achieves state-of-the-art performance with linear computational complexity. The effectiveness and efficiency of the SNN-ViT highlight its potential for power-critical edge vision applications.

==> trash <==
In ANNs, the self-attention mechanism effectively captures dependencies between any two positions within the input sequence, making it crucial for efficiently handling large-scale data. Let $\mathbf{X} \in \mathbb{R}^{n \times d}$ be the input to the self-attention block, where $n$ denotes the number of patches and $d$ is the embedding dimension. Initially, the input \(X\) is subjected to a layer normalization(LN) operation to ensure numerical stability throughout the model's training process. Then the Query, Key, and Value matrices are then derived as follows:


\begin{equation}
\mathbf{X'} = \mathbf{LN}(X), \quad \mathbf{Q} = \mathbf{X'}\mathbf{W}_{Q},  \quad \mathbf{K} = \mathbf{X'}\mathbf{W}_{K}, \quad \mathbf{V}= \mathbf{X'}\mathbf{W}_{V} 
\end{equation}

where $\mathbf{W}_{Q}, \mathbf{W}_{K}, \mathbf{W}_{V} \in \mathbb{R}$ represent the weight matrices. Then, the attention scores $\mathbf{S}$ are computed as:

\begin{equation}
\mathbf{Score} = \frac{\mathbf{Q} \mathbf{K}^{\top}}{\sqrt{d}}, \quad\mathbf{Z} = Softmax(\mathbf{Score}) \mathbf{V},
\end{equation}

$\mathbf{Score}$ are normalized using the $Softmax$ function, and the final self-attention output $\mathbf{Z}$ is obtained by $\mathbf{Score}$ and $\mathbf{V}$. 
